Diffractive Photoproduction of D*+/-(2010) at HERA

Diffractive photoproduction of D*+/-(2010) mesons was measured with the ZEUS detector at the ep collider HERA, using an integrated luminosity of 78.6 pb^{-1}. The D* mesons were reconstructed in the kinematic range: transverse momentum p_T(D*) > 1.9 GeV and pseudorapidity |eta(D*)| < 1.6, using the decay D*+ -> D0 pi+_s followed by D0 -> K- pi+ (+c.c.). Diffractive events were identified by a large gap in pseudorapidity between the produced hadronic state and the outgoing proton. Cross sections are reported for photon-proton centre-of-mass energies in the range 130 < W < 300 GeV and for photon virtualities Q^2 < 1 GeV^2, in two ranges of the Pomeron fractional momentum x_pom < 0.035 and x_pom < 0.01. The relative contribution of diffractive events to the inclusive D*+/-(2010) photoproduction cross section is about 6%. The data are in agreement with perturbative QCD calculations based on various parameterisations of diffractive parton distribution functions. The results are consistent with diffractive QCD factorisation.

==> com_def_tex.store/charm_com.tex <==
%
\newcommand{\ccb}        {\mbox{$c\bar{c}$}}
\newcommand{\bbb}        {\mbox{$b\bar{b}$}}
%
\newcommand{\ds}         {\mbox{$D^{\ast}$}}
\newcommand{\dsp}        {\mbox{$D^{\ast +}$}}
\newcommand{\dspm}       {\mbox{$D^{\ast \pm}$}}
%
\newcommand{\dss}        {\mbox{$D_s$}}
\newcommand{\dssp}       {\mbox{$D_s^+$}}
\newcommand{\dssn}       {\mbox{$D_s^-$}}
\newcommand{\dsspm}      {\mbox{$D_s^{\pm}$}}
%
\newcommand{\dsss}       {\mbox{$D_s^{\ast}$}}
\newcommand{\dsssp}      {\mbox{$D_s^{\ast +}$}}
\newcommand{\dsssn}      {\mbox{$D_s^{\ast -}$}}
\newcommand{\dssspm}     {\mbox{$D_s^{\ast \pm}$}}
%
\newcommand{\dz}         {\mbox{$D^{0}$}}
%
\newcommand{\dzs}        {\mbox{$D^{\ast 0}$}}
%
\newcommand{\dssz}       {\mbox{$D^{\ast \ast 0}$}}
%
\newcommand{\dspr}       {\mbox{$D^{\ast \prime \pm}$}}
\newcommand{\fcdpr}      {\mbox{$f(c \rightarrow D^{\ast \prime +})$}}
%
\newcommand{\dc}         {\mbox{$D^+$}}
\newcommand{\dcpm}       {\mbox{$D^{\pm}$}}
%
\newcommand{\lc}         {\mbox{$\Lambda_c$}}
\newcommand{\lcp}        {\mbox{$\Lambda_c^+$}}
\newcommand{\lcpm}       {\mbox{$\Lambda_c^\pm$}}
%
\newcommand{\xic}        {\mbox{$\Xi_c$}}
\newcommand{\omc}        {\mbox{$\Omega_c$}}
%
\newcommand{\dsone}      {\mbox{$D_{s 1}^{+}$}}
\newcommand{\dsonepm}    {\mbox{$D_{s 1}^{\pm}$}}
%
\newcommand{\done}       {\mbox{$D_1^{0}$}}
\newcommand{\dtwo}       {\mbox{$D_2^{\ast 0}$}}
%
\newcommand{\fcsone}     {\mbox{$f(c \rightarrow D_{s 1}^+)$}}
%
\newcommand{\fcdone}     {\mbox{$f(c \rightarrow D_1^0)$}}
\newcommand{\fcdtwo}     {\mbox{$f(c \rightarrow D_2^{\ast 0})$}}
%
\newcommand{\fcdz}       {\mbox{$f(c \rightarrow D^0)$}}
\newcommand{\fcdc}       {\mbox{$f(c \rightarrow D^+)$}}
\newcommand{\fcdss}      {\mbox{$f(c \rightarrow D_s^+)$}}
\newcommand{\fclc}       {\mbox{$f(c \rightarrow \Lambda_c^+)$}}
\newcommand{\fcds}       {\mbox{$f(c \rightarrow D^{\ast +})$}}
%
\newcommand{\fcdl}       {\mbox{$f(c \rightarrow D,\Lambda)$}}
%
\newcommand{\fcte}       {\mbox{$f(\bar{c} \rightarrow e^-)$}}
%
\def\dskpi{ {\dsp}~\rightarrow~\dz~\pi^{+}_{s}%
        \rightarrow~(K^{-}~\pi^{+})~\pi^{+}_{s} }
%
\def\dskspipi{ {\dsp}~\rightarrow~\dz~\pi^{+}_{s}%
        \rightarrow~(K^{0}_s~\pi^{+}\pi^{-})~\pi^{+}_{s} }
%
\def\dsk3pi{ {\dsp}~\rightarrow~\dz~\pi^{+}_{s}%
        \rightarrow~(K^{-}~\pi^{+}~\pi^{+}~\pi^{-})~\pi^{+}_{s} }
%
\def\dssphipi{ {\dssp}~\rightarrow~\phi~\pi^{+}%
        \rightarrow~(K^{-}~K^{+})~\pi^{+} }
%
\def\dzkpi{ {\dz}~\rightarrow~K^{-}~\pi^{+} }
%
\def\dpkpi{ {\dz}~\rightarrow~K^{-}~\pi^{+} }
%
\def\dckpipi{ {\dc}~\rightarrow~K^{-}~\pi^{+}~\pi^{+} }
%
\def\lcpkpi{ {\lcp}~\rightarrow~p~K^{-}~\pi^{+} }
%
%
\newcommand{\pt}       {\mbox{$P_{\perp}$}}
%
\newcommand{\ptds}       {\mbox{$P_{\perp}^{\ds}$}}
%
\newcommand{\ptdss}       {\mbox{$P_{\perp}^{\dss}$}}
%
\def\eten{ E_\perp^{\theta > 10^\circ}}
%
\def\et10t{ E_T^{\theta > 10^\circ}}
%
\def\ETJT{E_T^{\rm jet}}
%
\def\ETAJT{\eta^{\rm jet}}
%
\def\PHIJT{\phi^{\rm jet}}
%
\def\ptr{p_T^{\rm rel}}
%


==> com_def_tex.store/journal_def.tex <==
% A useful Journal macro
\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}

% Some useful journal names
\def\NCA{{\em Nuovo Cimento}}
\def\NIM{{\em Nucl. Instrum. Methods}}
\def\NIMA{{\em Nucl. Instrum. Methods} A}
\def\NPA{{\em Nucl. Phys.} A}
\def\NPB{{\em Nucl. Phys.} B}
\def\PLB{{\em Phys. Lett.}  B}
\def\PR{{\em Phys. Reports} }
\def\PRA{{\em Phys. Reports}  A}
\def\PRL{{\em Phys. Rev. Lett.} }
\def\PRD{{\em Phys. Rev.} D}
\def\ZPC{{\em Z. Phys.} C}
\def\EPC{{\em Eur. Phys. J.} C}
\def\CPC{{\em Comp. Phys. Comm.} }
\def\CNPP{{\em Comm. Nucl. Part. Phys.} }
%
\def\SJNP{{\em Sov. J. Nucl. Phys.} }
\def\CJPB{{\em Czech. J. Phys.} B}
\def\IJMA{{\em Int. J. Mod. Phys.} A}
\def\RMP{{\em Rev. Mod. Phys.} }
\def\FP{{\em Fortschr. Phys.} }
\def\ZP{{\em Z. Phys.} }
%


==> com_def_tex.store/journal_def_foster.tex <==
% A useful Journal macro
\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}

% Some useful journal names
\def\NCA{{\rm Nuovo Cimento}}
\def\NIM{{\rm Nucl. Instrum. Methods}}
\def\NIMA{{\rm Nucl. Instrum. Methods} A~}
\def\NPA{{\rm Nucl. Phys.} A~}
\def\NPB{{\rm Nucl. Phys.} B~}
\def\PLB{{\rm Phys. Lett.}  B~}
\def\PRA{{\rm Phys. Reports}  A~}
\def\PRL{{\rm Phys. Rev. Lett.} }
\def\PRD{{\rm Phys. Rev.} D~}
\def\ZPC{{\rm Z. Phys.} C~}
\def\EPC{{\rm Eur. Phys. J.} C~}
\def\CMC{{\rm Comp. Phys. Comm.} }
\def\CNPP{{\rm Comm. Nucl. Part. Phys.} }
%
\def\SJNP{{\rm Sov. J. Nucl. Phys.} }
\def\CJPB{{\rm Czech. J. Phys.} B~}
%


==> com_def_tex.store/newcom.tex <==
%
\newcommand{\GeVs}      {\mbox{${\rm GeV}^2$}}
\newcommand{\GeV}       {\mbox{${\rm GeV}$}}
\newcommand{\MeV}       {\mbox{${\rm MeV}$}}
\newcommand{\qsq}       {\mbox{${Q^2}$}}
\newcommand{\rhod}      {\mbox{${\rho^0}$}}
%\newcommand{\wgp}      {\mbox{${W_{\gamma p}}$}}
\newcommand{\wgp}       {\mbox{${W}$}}
\newcommand{\empz}      {\mbox{${\delta}$}}
\newcommand{\phid}      {\mbox{${\phi}$}}
\newcommand{\jpsid}     {\mbox{${J/\psi}$}}
\newcommand{\yjb}       {\mbox{${y_{_{JB}}}$}}
%
\newcommand{\ys}        {\mbox{$y_{\Sigma}$}}
\newcommand{\xes}       {\mbox{$x_{e\Sigma}$}}
\newcommand{\wes}       {\mbox{$W_{e\Sigma}$}}
\newcommand{\eda}       {\mbox{$E_{DA}^{\prime}$}}
%
\newcommand{\ra}        {\mbox{$\rightarrow$}}
\newcommand{\gsp}       {\mbox{$\gamma^* p$}}
\newcommand{\xda}       {\mbox{$x_{DA}$}}
\newcommand{\qda}       {\mbox{$Q^{2}_{DA}$}}
\newcommand{\qe}        {\mbox{$Q^{2}_{e}$}}
\newcommand{\gsubh}     {\mbox{$\gamma_{_{H}}$}}
\newcommand{\te}        {\mbox{$\theta_{e}^{\prime}$}}
\newcommand{\Ee}        {\mbox{$E_{e}^{\prime}$}}
\newcommand{\gh}        {\mbox{$\gamma_{h}$}}
\newcommand{\mrsdm}     {\mbox{MRSD$_-^{\prime}$\ }}
\newcommand{\mrsdz}     {\mbox{MRSD$_0^{\prime}$\ }}
\newcommand{\ftwo}      {\mbox{$F_{2}$}}
\newcommand{\ftwoccb}   {\mbox{$F_{2}^{c\bar c}$}}
%\newcommand{\ftwoccb}   {\mbox{$F_{2}^{c}$}}
\newcommand{\ptr}       {\mbox{$p_{T}$}}
\newcommand{\ccb}       {\mbox{$c\bar{c}$}}
\newcommand{\dspm}      {\mbox{$D^{\ast \pm}$}}
\newcommand{\ds}        {\mbox{$D^{\ast}$}}
\newcommand{\dz}        {\mbox{$D^{0}$}}
\newcommand{\mc}        {\mbox{$m_{c}$}}
\newcommand{\dm}        {\mbox{$\Delta M$}}
\newcommand{\dsp}       {\mbox{$D^{\ast +}$}}
\newcommand{\xd}        {\mbox{$x(D^{\ast})$}}
\newcommand{\ptds}      {\mbox{$p_T(D^{\ast})$}}
\newcommand{\etads}     {\mbox{$\eta(D^{\ast})$}}
\newcommand{\mkpi}      {\mbox{$M_{K\pi}$}}
\newcommand{\mdz}       {\mbox{$M(D^0)$}}
\newcommand{\mkpipis}   {\mbox{$M_{K\pi\pi_{s}}$}}
\newcommand{\ps}        {\mbox{$\pi_{s}$}}
\newcommand{\sleq} {\raisebox{-.6ex}{${\textstyle\stackrel{<}{\sim}}$}}
\newcommand{\sgeq} {\raisebox{-.6ex}{${\textstyle\stackrel{>}{\sim}}$}}
\renewcommand{\thefootnote}{\arabic{footnote}}
%


==> com_def_tex.store/physics_com.tex <==
%
\newcommand{\GeVs}      {\mbox{${\,\rm GeV}^2$}}
\newcommand{\GeV}       {\mbox{${\,\rm GeV}$}}
\newcommand{\MeV}       {\mbox{${\,\rm MeV}$}}
%
\newcommand{\sqs}       {\mbox{$\sqrt{s}$}}
\newcommand{\qsq}       {\mbox{${Q^2}$}}
%
\newcommand{\sig}       {\mbox{$\sigma$}}
\newcommand{\sigb}      {\mbox{$\sigma\cdot B$}}
%
\newcommand{\gcc}       {\mbox{$\Gamma_{c\bar c}$}}
\newcommand{\gha}       {\mbox{$\Gamma_{had}$}}
\newcommand{\gch}       {\mbox{$\frac{\Gamma_{c\bar c}}{\Gamma_{had}}$}}
\newcommand{\gchfb}     {\mbox{$\gch \cdot f(c\ra D,\Lambda) \cdot B$}}
%
\newcommand{\ga}        {\mbox{$\gamma$}}
\newcommand{\zn}        {\mbox{$\rm{Z}^0$}}
%
\newcommand{\gp}        {\mbox{$\gamma p$}}
%
\newcommand{\gaa}        {\mbox{$\gamma^{\ast}$}}
%
\newcommand{\gs}        {\mbox{$\gamma_s$}}
%
\newcommand{\Pom}       {\mbox{I$\!$P}}
%
\newcommand{\lum}{\mbox{$\cal L$}}
%pomeron in text
\newcommand {\pom} {I\!\!P}
%pomeron as subscript
\newcommand {\pomsub} {{\scriptscriptstyle \pom}}
\newcommand {\reg} {I\!\!R}
\newcommand {\regsub} {{\scriptscriptstyle \reg}}
\newcommand {\ppp} {\pom\pom\pom}
\newcommand {\ppr} {\pom\pom\reg}
\newcommand {\xpom} {x_{\pomsub}}
\newcommand {\zpom} {z_{\pomsub}}
\newcommand {\apom} {\alpha_{\pomsub}}
\newcommand {\areg} {\alpha_{\regsub}}
%
\newcommand {\as} {\alpha_s}
%
%
\newcommand {\qqb} {q\bar{q}}
%
\newcommand {\xgo} {\mbox{$x_{\gamma}^{\rm{OBS}}$}}
%


==> com_def_tex.store/physics_rus.tex <==
%
\newcommand{\rgevs}     {\mbox{$\,$Ĵ'$^2$}}
\newcommand{\rgev}      {\mbox{$\,$Ĵ'}}
\newcommand{\rmev}      {\mbox{$\,$δ'}}
%


==> com_def_tex.store/technic_com.tex <==
%
\newcommand{\tpm}        {\mbox{$\,\pm\,$}}
%
\newcommand{\ra}         {\mbox{$\rightarrow$}}
%


==> com_def_tex/journal_def_foster.tex <==
% A useful Journal macro
\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}

% Some useful journal names
\def\NCA{{\rm Nuovo Cimento}}
\def\NIM{{\rm Nucl. Instrum. Methods}}
\def\NIMA{{\rm Nucl. Instrum. Methods} A~}
\def\NPA{{\rm Nucl. Phys.} A~}
\def\NPB{{\rm Nucl. Phys.} B~}
\def\PLB{{\rm Phys. Lett.}  B~}
\def\PRA{{\rm Phys. Reports}  A~}
\def\PRL{{\rm Phys. Rev. Lett.} }
\def\PRD{{\rm Phys. Rev.} D~}
\def\ZPC{{\rm Z. Phys.} C~}
\def\EPC{{\rm Eur. Phys. J.} C~}
\def\CMC{{\rm Comp. Phys. Comm.} }
\def\CNPP{{\rm Comm. Nucl. Part. Phys.} }
%
\def\SJNP{{\rm Sov. J. Nucl. Phys.} }
\def\CJPB{{\rm Czech. J. Phys.} B~}
%


==> com_def_tex/newcom.tex <==
%
\newcommand{\GeVs}      {\mbox{${\rm GeV}^2$}}
\newcommand{\GeV}       {\mbox{${\rm GeV}$}}
\newcommand{\MeV}       {\mbox{${\rm MeV}$}}
\newcommand{\qsq}       {\mbox{${Q^2}$}}
\newcommand{\rhod}      {\mbox{${\rho^0}$}}
%\newcommand{\wgp}      {\mbox{${W_{\gamma p}}$}}
\newcommand{\wgp}       {\mbox{${W}$}}
\newcommand{\empz}      {\mbox{${\delta}$}}
\newcommand{\phid}      {\mbox{${\phi}$}}
\newcommand{\jpsid}     {\mbox{${J/\psi}$}}
\newcommand{\yjb}       {\mbox{${y_{_{JB}}}$}}
%
\newcommand{\ys}        {\mbox{$y_{\Sigma}$}}
\newcommand{\xes}       {\mbox{$x_{e\Sigma}$}}
\newcommand{\wes}       {\mbox{$W_{e\Sigma}$}}
\newcommand{\eda}       {\mbox{$E_{DA}^{\prime}$}}
%
\newcommand{\ra}        {\mbox{$\rightarrow$}}
\newcommand{\gsp}       {\mbox{$\gamma^* p$}}
\newcommand{\xda}       {\mbox{$x_{DA}$}}
\newcommand{\qda}       {\mbox{$Q^{2}_{DA}$}}
\newcommand{\qe}        {\mbox{$Q^{2}_{e}$}}
\newcommand{\gsubh}     {\mbox{$\gamma_{_{H}}$}}
\newcommand{\te}        {\mbox{$\theta_{e}^{\prime}$}}
\newcommand{\Ee}        {\mbox{$E_{e}^{\prime}$}}
\newcommand{\gh}        {\mbox{$\gamma_{h}$}}
\newcommand{\mrsdm}     {\mbox{MRSD$_-^{\prime}$\ }}
\newcommand{\mrsdz}     {\mbox{MRSD$_0^{\prime}$\ }}
\newcommand{\ftwo}      {\mbox{$F_{2}$}}
\newcommand{\ftwoccb}   {\mbox{$F_{2}^{c\bar c}$}}
%\newcommand{\ftwoccb}   {\mbox{$F_{2}^{c}$}}
\newcommand{\ptr}       {\mbox{$p_{T}$}}
\newcommand{\ccb}       {\mbox{$c\bar{c}$}}
\newcommand{\dspm}      {\mbox{$D^{\ast \pm}$}}
\newcommand{\ds}        {\mbox{$D^{\ast}$}}
\newcommand{\dz}        {\mbox{$D^{0}$}}
\newcommand{\mc}        {\mbox{$m_{c}$}}
\newcommand{\dm}        {\mbox{$\Delta M$}}
\newcommand{\dsp}       {\mbox{$D^{\ast +}$}}
\newcommand{\xd}        {\mbox{$x(D^{\ast})$}}
\newcommand{\ptds}      {\mbox{$p_T(D^{\ast})$}}
\newcommand{\etads}     {\mbox{$\eta(D^{\ast})$}}
\newcommand{\mkpi}      {\mbox{$M_{K\pi}$}}
\newcommand{\mdz}       {\mbox{$M(D^0)$}}
\newcommand{\mkpipis}   {\mbox{$M_{K\pi\pi_{s}}$}}
\newcommand{\ps}        {\mbox{$\pi_{s}$}}
\newcommand{\sleq} {\raisebox{-.6ex}{${\textstyle\stackrel{<}{\sim}}$}}
\newcommand{\sgeq} {\raisebox{-.6ex}{${\textstyle\stackrel{>}{\sim}}$}}
\renewcommand{\thefootnote}{\arabic{footnote}}
%

